DELTA: Dense Efficient Long-range 3D Tracking for any video

Tracking dense 3D motion from monocular videos remains challenging, particularly when aiming for pixel-level precision over long sequences. We introduce DELTA, a novel method that efficiently tracks every pixel in 3D space, enabling accurate motion estimation across entire videos. Our approach leverages a joint global-local attention mechanism for reduced-resolution tracking, followed by a transformer-based upsampler to achieve high-resolution predictions. Unlike existing methods, which are limited by computational inefficiency or sparse tracking, DELTA delivers dense 3D tracking at scale, running over 8x faster than previous methods while achieving state-of-the-art accuracy. Furthermore, we explore the impact of depth representation on tracking performance and identify log-depth as the optimal choice. Extensive experiments demonstrate the superiority of DELTA on multiple benchmarks, achieving new state-of-the-art results in both 2D and 3D dense tracking tasks. Our method provides a robust solution for applications requiring fine-grained, long-term motion tracking in 3D space.

==> figures/figure_teaser_arxiv.tex <==
\begin{figure}[th]
\centering
\includegraphics[width=\linewidth]{images/teaser16.pdf}
\captionof{figure}{
   % \textbf{a)} We introduce \Approach, the first dense 3D tracking approach, which can track every pixel of a video in 3D space in a feed-forward manner. Our model achieves SOTA results on 3D tracking benchmarks while significantly faster than previous tracking approaches in the dense setting \tuan{mention hardware + reso} on the same hardware and resolution. \textbf{Bottom:} We showcase our dense 3D trajectory estimations for \textit{in-the-wild} (first two rows) and \textit{AI-generated} videos (last row).
   \textbf{\Approach} is a dense 3D tracking approach that (a) tracks \textit{every} pixel from a monocular video, (b) provides consistent trajectories in 3D space, and (c) achieves state-of-the-art accuracy on 3D tracking benchmarks while being significantly faster than previous approaches in the dense setting.
   %, where we track all pixels of a 100-frame video with the resolution of $384 \times 512$, on a single A100 GPU.
   %\textbf{a)} We introduce \Approach, the first dense 3D tracking approach, which can track every pixel from a monocular video, \textbf{b)} achieving consistent trajectories in 3D space in a feed-forward manner. \textbf{c)} Our model achieves SOTA results on 3D tracking benchmarks while being significantly faster than previous tracking approaches in the dense setting, where we track all pixels of a 100-frame video with the resolution of $384 \times 512$, on a single A100 GPU.
}
\label{fig:teaser}
\end{figure}

==> figures/figures_flow2d.tex <==
\begin{figure}[t]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.98\linewidth]{images/compare_flow2d.pdf}
\caption{Comparison of long-range optical flow predictions: We predict optical flows from the first frame to subsequent frames of the video. DOT \citep{dot}, which lacks strong temporal correlation, suffers from a noticeable "flickering" effect (\textcolor{green}{green} circle), particularly at the boundaries between foreground and background objects. In contrast, our method ensures a smooth and consistent transition over time, effectively reducing artifacts at object boundaries.}
\end{center}
\label{fig:fig_compare_flow2d}
\end{figure}

==> figures/figures_qual_tap.tex <==
\begin{figure}[th]
\centering
\includegraphics[width=\linewidth]{images/quali2.pdf}
\captionof{figure}{
   Qualitative results of our method and SpatialTracker \citep{spatialtracker} on the TAP-Vid3D benchmark \citep{tapvid3d}. \textcolor{red}{Red} lines denote the groundtruth trajectories while \textcolor{green}{green} lines denote the predicted trajectories.
   \cwang{It is hard to tell whether our method is better/worse in the car example. } \tuan{maybe we move this to appendix}
}
\label{fig:quali}
\end{figure}

==> figures/figures_var_spaattn.tex <==
\begin{figure}[t]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.98\linewidth]{images/spaattn.pdf}
\caption{\textbf{Three different variants of spatial attention}. \textbf{\Circled[]{1}}: Vanilla self attention. \textbf{\Circled[]{2}}: Cotracker's spatial attention with a set of \textit{learnable tokens}. \textbf{\Circled[]{3}}: Our proposed spatial attention for dense prediction. \cwang{make this figure only about cross-attention, also draw illustration of cotracker's cross attention architecture of virtual tracks. so}}
\label{fig:decouple_spaattn}
\end{center}
\end{figure}

==> sections/3_method_backup.tex <==
\section{Method}
\label{sec:method}

Our goal is to track pixels of an in-the-wild video in 3D space. The tracking model must satisfy three criteria: 
\begin{itemize}
    \item long-term tracking (throughout a video of hundreds frames).
    \item dense (can track hundreds of thousands points in a single forward pass).
    \item provide 3D trajectories (in the camera space).
\end{itemize}

% We formulate the problem as: given a monocular video as input, we track all pixels from a query frame (usually first frame) throughout the video in 3D space in a single forward pass. 
In details, we take an input RGB video $\mV \in \mathbb{R}^{T \times H \times W \times 3}$ where $T$ is the video length, $H$ and $W$ are the video resolution, and its depth $\mD \in \mathbb{R}^{T \times H \times W \times 1}$ from an off-the-shelf monocular depth estimation, to predict a dense 3D trajectory set $\mP \in \mathbb{R}^{T \times (H \times W) \times 3}$, where $P_t^i = (u_t^i, v_t^i, d_t^i, o_t^i) \in \mathbb{R}^4, t = 1,\ldots, T, i = 1, \ldots, H \times W$ 
is the location and visible status of the $i$-th pixel of frame $0$-th at the $t$-th frame. Specifically, $(u_t^i, v_t^i)$ is the pixel coordinate, $d_t^i$ is the depth estimation and $o_t^i$ is the visibility prediction. For simplicity, we assume that we start tracking from the first frame of the video, and this can be easily generalized to tracking at any frame of the input video, so $t_0 \in \{1,T\}$. 

We build our method based on the sparse 2D tracking: CoTracker \citep{karaev2023cotracker} with transformer architecture. First, we incorporate a straightforward and effective modification on top of the architecture of CoTracker to obtain 3D trajectories (in Sec.~\ref{track3d}). Second, we introduce a novel technique to make CoTracker be able to track dense points in a single forward pass (in Sec.~\ref{track3d}). Finally, we introduce an inference strategy to obtain consistent dense 3D trajectories from multiple keyframes (in Sec.~\ref{track3d}).

\myheading{Overview.} Our proposed \Approach~architecture is illustrated in Fig. ~\ref{}. Our \Approach~contains an CNN-encoder to extract frame-wise feature maps from the input video. Then, a set of low-resolution dense 3D trajectories are initialized and refined through a transformer with spatial and temporal attentions. Lastly, the low-resolution dense 3D trajectories are passed through an attention-based upsampler to get the final high-resolution dense 3D trajectories.

% \subsection{Premilinary: CoTracker}

% CoTracker was initially introduced to tackle the task of sparse 2D tracking. It is a s

\subsection{Making CoTracker as 3D track}
\label{track3d}

We adopt the architecture of CoTracker \citep{karaev2023cotracker} for our 3D tracking approach. Unlike SpaTracker, which utilizes the 3D-triplane representation to directly track trajectories in 3D space, we operate in 2.5D space. In our approach, we supplement the transformer input with depth information and introduce an additional head to predict depth changes, alongside the existing predictions for 2D movement and visibility.

Following \cite{karaev2023cotracker,SpatialTracker}, we partition the video into overlapping windows of length $S$. We then iteratively estimate 3D trajectories for query points over $M$ refinement steps using a transformer. After each window, the estimated 3D trajectories are propagated and updated in the next window, continuing until the video’s end.

\myheading{Initializing 3D Trajectories:} For each query point $i$ at the initial frame, we start with its \textit{uv}-coordinates $(u_0^i, v_0^i)$ and use the estimated depth at the query frame to obtain the initial 3D point $\mathbf{P}0^i = (u_0^i, v_0^i, d_0^i, 1)$. We assume all points are visible in the first frame ($o_0^i = 1$ for all $i$). This 3D position is replicated across subsequent frames to initialize the 3D trajectory $\mathbf{P}^i{t=1,\ldots,S}$ of length $S$.

\myheading{Iterative Refinement:} We refine the initial 3D trajectory predictions iteratively within each temporal window. Let $\mathbf{X}^i_{(0)} = \mathbf{P}^i_{t=1,\ldots,S}$ represent the initial trajectory prediction, and after $m$ refinement steps, the refined trajectory is denoted as $\mathbf{X}^i_{(m)}$. As in \cite{karaev2023cotracker}, we encode these trajectories into tokens for the transformer module $\Phi$. For a query point $i$ at frame $t$ and iteration $m$, the input token is defined as:

\begin{equation}
G_t^m = [F_t^m, C_t^m, D_t^m, \gamma(X_t^m - X_1)] + \gamma_{pos}(X_t^m) + \gamma_{time}(t), \in \mathbb{R}^D, \quad (1)
\end{equation}

where:
\begin{itemize}
    \item $F_t^m$ is the track feature, queried from the feature map at the initial tracking position in the first frame.
    \item $C_t^m$ is the feature correlation \citep{teed2020raft, harley2022particle, karaev2023cotracker}, computed by comparing track features to image features around the current estimated track location.
    \item $D_t^m$ is the depth correlation, calculated as the difference between the current estimated depth and the depth queried from the depth map around the estimated track location.
    \item $\gamma_{pos}$ and $\gamma_{time}$ are the positional embedding of the input position and time frame, respectively.
\end{itemize}

The tokens are passed through the transformer $\Phi$ consisting six blocks of spatial-temporal attention layers to obtain the update signals. Each update computes the:
\begin{equation}
    \Delta (X_{uv}), \Delta (X_{d}), \Delta (F) = \Phi(G_t^m)
\end{equation}

thus we can update the trajectory by:
\begin{equation}
\label{eqn:update1}
    (X_{uv})_t^{m+1}=(X_{uv})_t^m + \Delta (X_{uv}), \quad(X_{d})_t^{m+1}=(X_{d})_t^m + \Delta (X_{d})
\end{equation}

\myheading{Depth Change Representation:} SpaTracker \citep{SpatialTracker} and SceneTracker \citep{wang2024scenetracker} choose to predict the delta depth as the depth change representation. However, we found that this desgin choice is ineffective. 
\begin{itemize}
    \item First, the depth range of videos in training and testing are significant different due to various scenario (we train on synthetic dataset (Kubric), and testing on in-the-wild videos). The delta depth is not scale-aware, causing gap between training and testing
    \item Second, given two objects, one near the camera plane, one further away, if both change the same amount of depth, the nearby objects will cause a larger visual effect to the captured video. And in real application, mostly we want the model to capture motion in nearby objects (usually foreground objects), rather than background. 
\end{itemize}

Based on these observations, we propose replacing delta depth prediction with ratio depth prediction. This new representation offers several advantages:

\begin{itemize}
    \item Sensitivity to nearby objects: Small changes in the absolute depth of proximal objects result in significant displacements in ratio depth, enhancing the model's ability to capture subtle movements.
    \item The model learns to focus on relative scale changes of objects over time rather than absolute depth changes. By learning relative depth changes, the model becomes less dependent on the specific depth ranges present in the training data. This characteristic enhances its performance when applied to in-the-wild videos, where depth ranges may vary considerably from those in the training set.
\end{itemize}

In practice we predict the ratio depth in the logarith space to facilitate the learning process. Thus, the update function in Eqn.~\ref{eqn:update1} becomes:

\begin{equation}
    (X_{uv})_t^{m+1}=(X_{uv})_t^m + \Delta (X_{uv}), \quad(X_{d})_t^{m+1}=(X_{d})_t^m * exp(logratio(X_{d}))
\end{equation}

where $\Delta (X_{uv})$ and $logratio(X_{d})$ are outputs from the transformer.

\subsection{Making Cotracker3D as dense 3D track}
In theory, our design allows for simultaneous tracking of $N=H \times W$ query points throughout the video. However, the spatial attention mechanism and correlation module exhibit quadratic memory growth relative to the number of query points, making it computationally infeasible to process hundreds of thousands of points concurrently. To address this limitation, previous approaches \citep{karaev2023cotracker, SpatialTracker} resort to dividing query points into chunks and tracking them sequentially. This method, while functional, proves inefficient (requiring approximately 30 minutes to 1 hour to generate a dense track map for a 100-frame video) and lacks coherence across tracks. Other approaches leverage dense optical flow \citep{teed2020raft} to initialize dense long-term track \citep{cho2024flowtrack} or to refine track \citep{lemoing2024dense}. Different from these approaches, we unify the dense long-term trajectory prediction into a single architecture, without any additional external models \citep{lemoing2024dense, cho2024flowtrack}, or separate predictions \citep{karaev2023cotracker}, with two novel designs:
\begin{itemize}
    \item Decoupling the spatial attention layer to get low-resolution dense 3D tracking.
    \item Introducing a learnable upsample layer to get high-resolution dense 3D tracking.
\end{itemize}

% Overall, we start tracking a set of low-resolution dense tracks of $N_l=H/4 \times W/4$ elements (corresponding to the 4-times downsampled image ($H/4 \times W/4)$) using iterative refinements using the transformer with our decouple spatial attention. After obtaining the low-resolution dense 3D tracking map $\mathbf{L} \in \mathbb{R}^{(T \times N_l \times 3)}$, we apply the attention-based upsample layer to obtain the high-resolution dense tracking map $\mathbf{L} \in \mathbb{R}^{(T \times N_h \times 3)}$, where $N_h = H \times W$. 

Our tracking process begins with a set of low-resolution dense tracks comprising $N_l = H/4 \times W/4$ elements, corresponding to a 4-times downsampled version of the original image ($H \times W$). We iteratively refine these tracks using a transformer equipped with our novel decoupled spatial attention mechanism. This initial step yields a low-resolution dense 3D tracking map $\mathbf{L}_l \in \mathbb{R}^{T \times N_l \times 3}$, where $T$ represents the temporal dimension.
To achieve full resolution, we subsequently apply an attention-based upsampling layer. This operation transforms the low-resolution map into a high-resolution dense tracking map $\mathbf{L}_h \in \mathbb{R}^{T \times N_h \times 3}$, where $N_h = H \times W$, matching the original image dimensions. This two-stage approach—initial low-resolution tracking followed by intelligent upsampling—allows us to balance computational efficiency with high-fidelity tracking results.

\subsubsection{Decoupling Spatial Attention}
Our transformer $\Phi$ consists of interleave spatial-temporal attention operators that operate across the time and track dimensions, respectively. The complexity is $O(N^2 + T^2)$. In CoTracker \citep{karaev2023cotracker}, they introduce K virtual tracking tokens which can reduce the complexity of the transformer to $O(NK + K^2 + T^2)$. However, even with this design, when training with a modern GPU (A100 with 80G of memory) the model cannot fit a large number of query points (~100K) at the same time. Thus, in our approach, we further decouple the spatial attention into several layers of cross attention and self attention. 

The virtual track tokens are a set of learnable embedding which are randomly initialized at the beginning of the training. They participate in the spatial attention.

\begin{itemize}
    \item First, we do the cross-attention between the $K$ virtual track tokens ($\mathbf{Q}$) with the set of $N$ sparse tracks ($\mathbf{K}$, $\mathbf{V}$). 
    \item Second, the virtual tracks are passing through the self-attention.
    \item Finally, we do cross-attention between the dense 3D tracks with the set of virtual tokens.
\end{itemize}



% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.90\linewidth]{images/decouple_spaattn.pdf}
%    \caption{\textbf{Decouple Spatial Attention Layer}. \tuan{Placeholde re-draw}}
%    \label{fig:decouple_spaattn}
% \end{figure*}

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
% \includegraphics[width=0.90\linewidth]{images/decouple_spaattn}
\includegraphics[width=0.90\linewidth]{images/decouple_spaattn.png}
\caption{\textbf{Decouple Spatial Attention Layer}. \tuan{Placeholde re-draw}}
\label{fig:decouple_spaattn}
\end{center}
\end{figure}

\subsubsection{Attention-based Upsample Layer}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.90\linewidth]{images/attn_upsampler.png}
\caption{\textbf{Attention Upsample Layer}. \tuan{Placeholde re-draw}}
\label{fig:attn_upsampler}
\end{center}
\end{figure}


A naive approach to obtain the high-resolution dense 3D tracks is using interpolation or averaging nearest neighbors in the 3D space of every pixel in the high-resolution image with its neighbors in the low-resolution image. However, these approach are suboptimal.

We leverage the attention mechanism to upsample the low-resolution dense 3D tracks. Inspired by \cite{hassani2023neighborhood}, we apply the attention in a local neighborhood region. To obtain the 3D trajectory of a pixel $i$ at $(u,v)$-location in the original image with resolution of $H \times W$, we first locate its nearest pixel in the low-resolution map by $(\lfloor u/4 \rfloor,\lfloor v/4 \rfloor)$, then we define a local region $\{\rho_{1},\ldots, \rho_{k\times k}\}$ of size $k \times k$ around this pixel. Let denote $Q,K,V$ as the query, key, value's linear projection, and $B_{(i,\rho_k(i))}$ as the relative positional bias \citep{alibi}. We can calculate the attention map of each point in the high-resolution map with its $9 \times 9$ neighbors in the low-resolution map as:

\begin{align}
\mathbf{A}i^k &= \begin{bmatrix}
Q_i K{\rho_1(i)}^T + B_{(i,\rho_1(i))} \\
Q_i K_{\rho_2(i)}^T + B_{(i,\rho_2(i))} \\
\vdots \\
Q_i K_{\rho_k(i)}^T + B_{(i,\rho_k(i))}
\end{bmatrix}\\
\end{align}

where $\rho_j(i)$ denotes $i$'s $j$-th nearest neighbor. We then define neighboring values, $\mathbf{V}_i^k$, as a matrix whose rows are the $i$-th input's $k$ nearest neighboring value projections:

\begin{equation}
    \mathbf{V}i^k = \begin{bmatrix}
V{\rho_1(i)}^T & V_{\rho_2(i)}^T & \cdots & V_{\rho_k(i)}^T
\end{bmatrix}^T
\end{equation}

Neighborhood Attention for the $i$-th token with neighborhood size $k$ is then defined as:

\begin{equation}
    \text{NA}_k(i) = \text{softmax}\left(\frac{\mathbf{A}_i^k}{\sqrt{d}}\right)\mathbf{V}_i^k
\end{equation}

where $\sqrt{d}$ is the scaling parameter. This operation is repeated for every pixel in the high-resolution feature map. Finally, the feature vector of each pixel in the high-resolution map is passed through an MLP to predict the $k \times k$ weights to average the tracks from $k \times k$ neighbors in the low-resolution track map.


\subsubsection{Forward-Backward Consistency}
Tracking solely from the first frame of a long video may not be sufficient for downstream applications, especially as the camera moves over time. As a result, some regions may become occluded or disappear, while new regions emerge in subsequent frames. In practice, it is desirable to generate dense 3D tracking maps from multiple keyframes and combine them to create a holistic, comprehensive map. However, tracking an object from multiple keyframes may introduce inconsistencies. This issue becomes even more pronounced in the 3D setting, where depth estimates are often inconsistent \citep{luo2020consistent, kopf2021robust}, exacerbating the challenge of maintaining 3D tracking consistency, even in static camera scenarios.

Assume that we want to track a video of 100 frames and the window size of each local chunk is 16. 

\subsection{Training}
\label{training}
We leverage Kubric simulation \citep{greff2021kubric} to generate 5632 training videos and 143 testing videos featuring rigid objects falling against diverse backgrounds, complete with ground-truth depths and dense 3D trajectory annotations. To expand the training set, we derive dense trajectories from the first, middle, and last frames of each video, effectively tripling the sample size. Following \cite{karaev2023cotracker, SpatialTracker}, we apply on-the-fly spatial and color augmentation, depth noising during training to further enhance diversity. We supervised the model on both sparse predictions (output directly from the transformer) and dense predictions (from the upsample layers) at every iteration. The total loss is defined as:
\begin{equation}
    \mathcal{L} = \lambda_{2d} \mathcal{L}_{2D} + \lambda_{depth}\mathcal{L}_{depth} + \lambda_{visib} \mathcal{L}_{visib} 
\end{equation}
where $\mathcal{L}_{2D}$ is the L1 loss between the 2D coordinate predictions and ground-truth, $\mathcal{L}_{depth}$ is the L1 loss of the inverse depth prediction and the inverse ground-truth depth, $\mathcal{L}_{visib}$ is the binary cross entropy loss.


\comment{
SpatialTracker \citep{spatialtracker} and SceneTracker \citep{scenetracker} choose to predict the delta depth as the depth change representation. However, we found that this desgin choice is ineffective. 
\begin{itemize}
    \item First, the depth range of videos in training and testing are significant different due to various scenario (we train on synthetic dataset (Kubric), and testing on in-the-wild videos). The delta depth is not scale-aware, causing gap between training and testing
    \item Second, given two objects, one near the camera plane, one further away, if both change the same amount of depth, the nearby objects will cause a larger visual effect to the captured video. And in real application, mostly we want the model to capture motion in nearby objects (usually foreground objects), rather than background. 
\end{itemize}

Based on these observations, we propose replacing delta depth prediction with ratio depth prediction. This new representation offers several advantages:

\begin{itemize}
    \item Sensitivity to nearby objects: Small changes in the absolute depth of proximal objects result in significant displacements in ratio depth, enhancing the model's ability to capture subtle movements.
    \item The model learns to focus on relative scale changes of objects over time rather than absolute depth changes. By learning relative depth changes, the model becomes less dependent on the specific depth ranges present in the training data. This characteristic enhances its performance when applied to in-the-wild videos, where depth ranges may vary considerably from those in the training set.
\end{itemize}

In practice we predict the ratio depth in the logarith space to facilitate the learning process. Thus, the update function in Eqn.~\ref{eqn:update1} becomes:

\begin{equation}
    (X_{uv})_t^{m+1}=(X_{uv})_t^m + \Delta (X_{uv}), \quad(X_{d})_t^{m+1}=(X_{d})_t^m * exp(logratio(X_{d}))
\end{equation}

where $\Delta (X_{uv})$ and $logratio(X_{d})$ are outputs from the transformer.




We design our model such a way to address the following challenges for dense 3D tracking:\\
\emph{Stable long-term 3D tracking} \\
\emph{}
\emph{Computational efficient} \\


\begin{itemize}
    \item long-term tracking (throughout a video of hundreds frames).
    \item dense (can track hundreds of thousands points in a single forward pass).
    \item provide 3D trajectories (in the camera space).
\end{itemize}

%For simplicity, we assume that we start tracking from the first frame of the video, and this can be easily generalized to tracking at any frame of the input video, so $t_0 \in \{1,T\}$. 

We build our method based on the sparse 2D tracking: CoTracker \citep{cotracker} with transformer architecture. First, we incorporate a straightforward and effective modification on top of the architecture of CoTracker to obtain 3D trajectories (in Sec.~\ref{track3d}). Second, we introduce a novel technique to make CoTracker be able to track dense points in a single forward pass (in Sec.~\ref{track3d}). Finally, we introduce an inference strategy to obtain consistent dense 3D trajectories from multiple keyframes (in Sec.~\ref{track3d}).

Specifically, : 


\myheading{Overview.} Our proposed \Approach~architecture is illustrated in Fig. ~\ref{}. Our \Approach~contains an CNN-encoder to extract frame-wise feature maps from the input video. Then, a set of low-resolution dense 3D trajectories are initialized and refined through a transformer with spatial and temporal attentions. Lastly, the low-resolution dense 3D trajectories are passed through an attention-based upsampler to get the final high-resolution dense 3D trajectories.

% \subsection{Premilinary: CoTracker}

% CoTracker was initially introduced to tackle the task of sparse 2D tracking. It is a s

\subsection{Making CoTracker as 3D track}
\label{track3d}

We adopt the architecture of CoTracker \citep{cotracker} for our 3D tracking approach. Unlike SpaTracker, which utilizes the 3D-triplane representation to directly track trajectories in 3D space, we operate in 2.5D space. In our approach, we supplement the transformer input with depth information and introduce an additional head to predict depth changes, alongside the existing predictions for 2D movement and visibility.

Following \cite{cotracker,spatialtracker}, we partition the video into overlapping windows of length $S$. We then iteratively estimate 3D trajectories for query points over $M$ refinement steps using a transformer. After each window, the estimated 3D trajectories are propagated and updated in the next window, continuing until the video’s end.

\myheading{Initializing 3D Trajectories:} For each query point $i$ at the initial frame, we start with its \textit{uv}-coordinates $(u_0^i, v_0^i)$ and use the estimated depth at the query frame to obtain the initial 3D point $\mathbf{P}0^i = (u_0^i, v_0^i, d_0^i, 1)$. We assume all points are visible in the first frame ($o_0^i = 1$ for all $i$). This 3D position is replicated across subsequent frames to initialize the 3D trajectory $\mathbf{P}^i{t=1,\ldots,S}$ of length $S$.

\myheading{Iterative Refinement:} We refine the initial 3D trajectory predictions iteratively within each temporal window. Let $\mathbf{X}^i_{(0)} = \mathbf{P}^i_{t=1,\ldots,S}$ represent the initial trajectory prediction, and after $m$ refinement steps, the refined trajectory is denoted as $\mathbf{X}^i_{(m)}$. As in \cite{cotracker}, we encode these trajectories into tokens for the transformer module $\Phi$. For a query point $i$ at frame $t$ and iteration $m$, the input token is defined as:

\begin{equation}
G_t^m = [F_t^m, C_t^m, D_t^m, \gamma(X_t^m - X_1)] + \gamma_{pos}(X_t^m) + \gamma_{time}(t), \in \mathbb{R}^D, \quad (1)
\end{equation}



The tokens are passed through the transformer $\Phi$ consisting six blocks of spatial-temporal attention layers to obtain the update signals. Each update computes the:
\begin{equation}
    \Delta (X_{uv}), \Delta (X_{d}), \Delta (F) = \Phi(G_t^m)
\end{equation}

thus we can update the trajectory by:
\begin{equation}
\label{eqn:update1}
    (X_{uv})_t^{m+1}=(X_{uv})_t^m + \Delta (X_{uv}), \quad(X_{d})_t^{m+1}=(X_{d})_t^m + \Delta (X_{d})
\end{equation}

\myheading{Depth Change Representation:} SpatialTracker \citep{spatialtracker} and SceneTracker \citep{scenetracker} choose to predict the delta depth as the depth change representation. However, we found that this desgin choice is ineffective. 
\begin{itemize}
    \item First, the depth range of videos in training and testing are significant different due to various scenario (we train on synthetic dataset (Kubric), and testing on in-the-wild videos). The delta depth is not scale-aware, causing gap between training and testing
    \item Second, given two objects, one near the camera plane, one further away, if both change the same amount of depth, the nearby objects will cause a larger visual effect to the captured video. And in real application, mostly we want the model to capture motion in nearby objects (usually foreground objects), rather than background. 
\end{itemize}

Based on these observations, we propose replacing delta depth prediction with ratio depth prediction. This new representation offers several advantages:

\begin{itemize}
    \item Sensitivity to nearby objects: Small changes in the absolute depth of proximal objects result in significant displacements in ratio depth, enhancing the model's ability to capture subtle movements.
    \item The model learns to focus on relative scale changes of objects over time rather than absolute depth changes. By learning relative depth changes, the model becomes less dependent on the specific depth ranges present in the training data. This characteristic enhances its performance when applied to in-the-wild videos, where depth ranges may vary considerably from those in the training set.
\end{itemize}

In practice we predict the ratio depth in the logarith space to facilitate the learning process. Thus, the update function in Eqn.~\ref{eqn:update1} becomes:

\begin{equation}
    (X_{uv})_t^{m+1}=(X_{uv})_t^m + \Delta (X_{uv}), \quad(X_{d})_t^{m+1}=(X_{d})_t^m * exp(logratio(X_{d}))
\end{equation}

where $\Delta (X_{uv})$ and $logratio(X_{d})$ are outputs from the transformer.



\subsection{Making Cotracker3D as dense 3D track}
In theory, our design allows for simultaneous tracking of $N=H \times W$ query points throughout the video. However, the spatial attention mechanism and correlation module exhibit quadratic memory growth relative to the number of query points, making it computationally infeasible to process hundreds of thousands of points concurrently. To address this limitation, previous approaches \citep{cotracker, spatialtracker} resort to dividing query points into chunks and tracking them sequentially. This method, while functional, proves inefficient (requiring approximately 30 minutes to 1 hour to generate a dense track map for a 100-frame video) and lacks coherence across tracks. Other approaches leverage dense optical flow \citep{raft} to initialize dense long-term track \citep{flowtrack} or to refine track \citep{dot}. Different from these approaches, we unify the dense long-term trajectory prediction into a single architecture, without any additional external models \citep{dot, flowtrack}, or separate predictions \citep{cotracker}, with two novel designs:
\begin{itemize}
    \item Decoupling the spatial attention layer to get low-resolution dense 3D tracking.
    \item Introducing a learnable upsample layer to get high-resolution dense 3D tracking.
\end{itemize}

% Overall, we start tracking a set of low-resolution dense tracks of $N_l=H/4 \times W/4$ elements (corresponding to the 4-times downsampled image ($H/4 \times W/4)$) using iterative refinements using the transformer with our decouple spatial attention. After obtaining the low-resolution dense 3D tracking map $\mathbf{L} \in \mathbb{R}^{(T \times N_l \times 3)}$, we apply the attention-based upsample layer to obtain the high-resolution dense tracking map $\mathbf{L} \in \mathbb{R}^{(T \times N_h \times 3)}$, where $N_h = H \times W$. 

Our tracking process begins with a set of low-resolution dense tracks comprising $N_l = H/4 \times W/4$ elements, corresponding to a 4-times downsampled version of the original image ($H \times W$). We iteratively refine these tracks using a transformer equipped with our novel decoupled spatial attention mechanism. This initial step yields a low-resolution dense 3D tracking map $\mathbf{L}_l \in \mathbb{R}^{T \times N_l \times 3}$, where $T$ represents the temporal dimension.
To achieve full resolution, we subsequently apply an attention-based upsampling layer. This operation transforms the low-resolution map into a high-resolution dense tracking map $\mathbf{L}_h \in \mathbb{R}^{T \times N_h \times 3}$, where $N_h = H \times W$, matching the original image dimensions. This two-stage approach—initial low-resolution tracking followed by intelligent upsampling—allows us to balance computational efficiency with high-fidelity tracking results.

\subsubsection{Decoupling Spatial Attention}

Due to the quadratic memory growth with respect to the number of query points, the architectures of SpaTracker and SceneTracker become computationally infeasible for processing hundreds of thousands of points simultaneously. One alternative is to replace spatial attention with a fully convolutional design \citep{dot} or eliminate spatial relationships between query points entirely \citep{cho2024local}. However, without robust correlations between query points across different regions of the frame, these methods deliver suboptimal results, particularly in the presence of significant camera motion (Fig.~\ref{fig:compare_spaattn}).


Our transformer $\Phi$ consists of interleave spatial-temporal attention operators that operate across the time and track dimensions, respectively. The complexity is $O(N^2 + T^2)$. In CoTracker \citep{cotracker}, they introduce K virtual tracking tokens which can reduce the complexity of the transformer to $O(NK + K^2 + T^2)$. However, even with this design, when training with a modern GPU (A100 with 80G of memory) the model cannot fit a large number of query points (~100K) at the same time. Thus, in our approach, we further decouple the spatial attention into several layers of cross attention and self attention. 

The virtual track tokens are a set of learnable embedding which are randomly initialized at the beginning of the training. They participate in the spatial attention.

\begin{itemize}
    \item First, we do the cross-attention between the $K$ virtual track tokens ($\mathbf{Q}$) with the set of $N$ sparse tracks ($\mathbf{K}$, $\mathbf{V}$). 
    \item Second, the virtual tracks are passing through the self-attention.
    \item Finally, we do cross-attention between the dense 3D tracks with the set of virtual tokens.
\end{itemize}



% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.90\linewidth]{images/decouple_spaattn.pdf}
%    \caption{\textbf{Decouple Spatial Attention Layer}. \tuan{Placeholde re-draw}}
%    \label{fig:decouple_spaattn}
% \end{figure*}

\input{figures/figures_var_spaattn}


\subsubsection{Attention-based Upsample Layer}


After the transformer part, we obtain a dense low-resolution 3D trajectories along with a refined feature vector of each trajectory. We borrow the \textit{convex upsample} in RAFT \cite{raft} to get the dense high-resolution 3d tracks with modification. The high level is the trajectory of each pixel $i$ in the high-resolution is the weighted sum of trajectories of a $k \times k$ region in the low-resolution map. The $k \times k$ region includes the nearest pixel of $i$ in the low-resolution map and $k \times k - 1$ adjacent pixels. To predict the weight, we apply the attention mechanism. The \textit{query} is the pixel $i$ in the high-resolution map while the \textit{key} and \textit{value} are $k \times k$ corresponding pixels in the low-resolution map.

In practice, we first add a CNN-decoder block (similar to \cite{esser2021taming}) to get the high-resolution feature map $\mathbf{F}_{hr}$. For every pixel $i$ at $(u,v)$-location in the original image with resolution of $H \times W$, we first locate its nearest pixel in the low-resolution map by $(\lfloor u/4 \rfloor,\lfloor v/4 \rfloor)$, then we concatenate the feature vector $\mathbf{F}_{hr}[u, v]$ with the tracking $\mathbf{X}_{lr}[\lfloor u/4 \rfloor,\lfloor v/4 \rfloor]$ to get the \textit{query} feature $\mathbf{J}_{i}$. Similarly, we concatenate the trajectory and feature vector of low-resolution pixels to obtain the $\mathbf{H}_{\rho_j(i)}$, where $\rho_j(i)$ denotes  $i$'s $j$-th nearest neighbor. Then the attention map of $i$ is calculated as:

\begin{align}
\mathbf{A}_i &= \begin{bmatrix}
Q(\mathbf{J}_{i}) K(\mathbf{H}_{\rho_1(i)})^T + \text{Alibi}(i, \rho_1(i))\\
Q(\mathbf{J}_{i}) K(\mathbf{H}_{\rho_2(i)})^T + \text{Alibi}(i, \rho_2(i))\\
\vdots \\
Q(\mathbf{J}_{i}) K(\mathbf{H}_{\rho_{k \times k}(i)})^T + \text{Alibi}(i, \rho_{k \times k}(i))
\end{bmatrix}\\
\mathbf{V}_{i} &= \begin{bmatrix} V(\mathbf{H}_{\rho_1(i)}), V(\mathbf{H}_{\rho_2(i)}), \ldots, V(\mathbf{H}_{\rho_{k \times k}(i)}) \end{bmatrix}
\end{align}

where $Q,K,V$ as the query, key, value's linear projection, $\text{Alibi}(,)$ is the relative positional bias \citep{alibi}. Then the local attention for the $i$-th pixel with its neighborhood size $k \times k$ in the low-resolution map is defined as::

\begin{equation}
    LocalAttn_{i} = softmax\left(\frac{\mathbf{A}_i}{\sqrt{s}}\right)\mathbf{V}_i^T
\end{equation}

where $s$ is a scaling parameter. This operation is repeated for every pixel in the high-resolution feature map and we apply several layer of \textit{local attention}. Finally, the feature vector of each pixel in the high-resolution map is passed through an MLP to predict the $k \times k$ weights to average the tracks from $k \times k$ neighbors in the low-resolution track map.


% \subsubsection{Forward-Backward Consistency}
% Tracking solely from the first frame of a long video may not be sufficient for downstream applications, especially as the camera moves over time. As a result, some regions may become occluded or disappear, while new regions emerge in subsequent frames. In practice, it is desirable to generate dense 3D tracking maps from multiple keyframes and combine them to create a holistic, comprehensive map. However, tracking an object from multiple keyframes may introduce inconsistencies. This issue becomes even more pronounced in the 3D setting, where depth estimates are often inconsistent \citep{luo2020consistent, kopf2021robust}, exacerbating the challenge of maintaining 3D tracking consistency, even in static camera scenarios.

% Assume that we want to track a video of 100 frames and the window size of each local chunk is 16. 

\subsection{Training}
\label{training}
We leverage Kubric simulation \citep{kubric} to generate 5632 training videos and 143 testing videos featuring rigid objects falling against diverse backgrounds, complete with ground-truth depths and dense 3D trajectory annotations. To expand the training set, we derive dense trajectories from the first, middle, and last frames of each video, effectively tripling the sample size. Following \cite{cotracker, spatialtracker}, we apply on-the-fly spatial and color augmentation, depth noising during training to further enhance diversity. We supervised the model on both sparse predictions (output directly from the transformer) and dense predictions (from the upsample layers) at every iteration. The total loss is defined as:
\begin{equation}
     \lambda_{2d} \mathcal{L}_{2D} + \lambda_{depth}\mathcal{L}_{depth} + \lambda_{visib} \mathcal{L}_{visib} 
\end{equation}
where $\mathcal{L}_{2D}$ is the L1 loss between the 2D coordinate predictions and ground-truth, $\mathcal{L}_{depth}$ is the L1 loss of the inverse depth prediction and the inverse ground-truth depth, $\mathcal{L}_{visib}$ is the binary cross entropy loss.
}



==> tables/table_ablation_1.tex <==
\begin{table}[ht]
    \begin{minipage}{0.45\linewidth}
        \setlength{\tabcolsep}{2pt}
       \begin{tabular}{cc|cc}
        \toprule
        \multirow{2}{*}{\textbf{Depth Rep.}} & \multirow{2}{*}{\textbf{Output}} & \multicolumn{2}{c}{\textbf{TAP-Vid3D} (\textit{Avg.})} \\
        & & AJ$\uparrow$ & APD$_{3D}\uparrow$ \\
        \midrule
        $d$ & $d_t - d_1$ & 9.0 & 15.0 \\
        $1/d$ & $1/d_t - 1/d_1$ & 9.4 & 15.6 \\
        $\log(d)$ & $\log(d_t/d_1)$ &\textbf{13.0 }& \textbf{20.3} \\
        \bottomrule
        \end{tabular}
        \caption{Ablation of different depth representations on the TAP-Vid3D benchmark.}
        \label{tab:ablation_depth}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        % \begin{tabular}{l|cc}
        % \toprule
        % \multirow{2}{*}{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{CVO}}  \\
        %  & EPE $\downarrow$  & OA $\uparrow$ \\
        % \midrule
        % Bilinear Up & 2.06 / 1.51 / 5.33 \\
        % NN Up & 2.05 / 1.50 / 5.20 \\
        % 3D KNN & 1.52 / 1.03 / 4.32 \\ 
        % \midrule
        % ConvUp & 1.15 / 0.66 / 3.83  \\
        % AttentionUp & x \\
        % AttentionUp + Alibi & 0.89 / 0.46 / 2.98 & 78.2 \\
        % \bottomrule
        % \end{tabular}
        % \caption{Ablation of different designs of the Upsampler}
        % \label{tab:ablation_upsampler}
        \setlength{\tabcolsep}{2pt}
        \begin{tabular}{cccc}
        %\setlength{\tabcolsep}{4pt}
        \toprule
        \textbf{GA} & \textbf{LA} & EPE$\downarrow$& OA$\uparrow$ \\
        \midrule
        & & 2.39 / 1.35 / 7.77 & 63.2\\
         & \checkmark & 1.79 / 1.13 / 5.24 & 75.1 \\
        \textit{back-and-forth} & & x \\
        \textit{1-ways} & & 0.94 / 0.49 / 3.09 & 78.1 \\
        \textit{1-ways} & \checkmark & 0.89 / 0.46 / 2.96 & 78.3 \\
        
        \bottomrule
        \end{tabular}
        \vspace{-4pt}
        \caption{Ablation on different designs of the Spatial Attention}
        \label{tab:ablation_spaattn}
    \end{minipage}

\end{table}


% \begin{table}
% \small
% \setlength{\tabcolsep}{4.5pt}
% \centering
% \begin{tabular}{cccc}
% \toprule
% \textbf{Attn with Virtual} & \textbf{Local Attn} & EPE$\downarrow$& OA$\uparrow$ \\
% \midrule
% & & 2.39 / 1.35 / 7.77 & 63.2\\
% \checkmark (2-ways) & & x \\
% \checkmark (1-ways & & 0.94 / 0.49 / 3.09 & 78.1 \\
%  & \checkmark & 1.79 / 1.13 / 5.24 & 75.1 \\
% \checkmark (1-ways) & \checkmark & 0.89 / 0.46 / 2.96 & 78.3 \\

% \bottomrule
% \end{tabular}
% \vspace{-4pt}
% \caption{Ablation on different designs of the Spatial Attention}
% \label{tab:ablation_components}
% \vspace{-4pt}
% \end{table}

==> tables/table_ablation_2.tex <==
\begin{table}
\centering
\small
\begin{tabular}{l|ccc}
\toprule
\multirow{2}{*}{\textbf{Setting}} & \multicolumn{2}{c}{\textbf{CVO}} \\
 & EPE $\downarrow$ & OA $\uparrow$ \\
\midrule
Without Spatial Attention & 2.39 / 1.35 / 7.77 & 63.2  \\
Only LocalAttention & 1.79 / 1.13 / 5.24 & 75.1  \\
Vanilla Spatial Attention & \multicolumn{2}{c}{\textit{---Out of memory---}}  \\
Decouple Spatial Attention (cross-attn with latent) & 0.94 / 0.49 / 3.09 \\
Decouple Spatial Attention (no cross-attn with latent) & 0.94 / 0.49 / 3.09 & 78.1 \\
Decouple Spatial Attention + LocalAttention & \textbf{0.89 } / \textbf{0.46} / \textbf{2.96} & \textbf{78.3} \\
\bottomrule
\end{tabular}
\caption{Ablation of different design of the Spatial Attention}
\end{table}
